Symmetries of colored Khovanov-Rozansky homology

We construct an action of the positive half of the Witt algebra on colored $\mathfrak{gl}_N$-Khovanov-Rozansky homology and prove that this action is compatible with the functoriality of colored link homology. To establish this result, we use Bar-Natan's framework of canopolies to formulate and prove the relevant statements at the level of tangles.

==> sch/def_dots_black_blank.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  % \filldraw[draw= black, fill = black] (A) circle (.7mm)
  % node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k P_{n-k}$};
\end{scope}


==> sch/def_dots_circle_black.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= black, fill = black] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
\end{scope}

==> sch/def_dots_circle_black_k.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= black, fill = black] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k P_{n-k}$};
\end{scope}

==> sch/def_dots_circle_hollow_k.tex <==

\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= \crd, fill = white] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k \deco_{n-k}$};
\end{scope}

==> sch/def_dots_circle_solid_k.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= \crd, fill = \csrd] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k \hat{\deco}_{n-k}$};
\end{scope}

==> sch/def_dots_trian_hollow_n.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A); 
  \node (C) at (0.5,0.7) [draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=1.5pt]{};
  \node (D) at (0.5,0.7) [below,yshift=-0.5mm]{$\omega$}; 
  \node (B) at (.55,.3) {$\deco_n$};
\end{scope}

==> sch/def_dots_trian_solid.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A); 
  \node (C) at (0.5,0.7) [draw=\crd, fill=\csrd,regular polygon, regular polygon sides=3,inner sep=1.5pt]{};
  \node (D) at (0.5,0.7) [below,  yshift=-0.5mm]{$\lambda$};   
\end{scope}

==> sch/def_dots_trian_solid_n.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A); 
  \node (C) at (0.5,0.7) [draw=\crd, fill=\csrd,regular polygon, regular polygon sides=3,inner sep=1.5pt]{};
  \node (D) at (0.5,0.7) [below]{$\lambda$};   
  \node (B) at (.55,.3) {$\hat{\deco}_n$};
\end{scope}

==> sch/ex_comp_plan_2.tex <==
\begin{scope}[yshift=-3,xshift=-15,rotate=80,font=\tiny]
    \draw[dotted] (.6,-0.1) circle (.25);
    \node (a) at (0.85,-0.1) {$*$};
    \draw[] (.403, .059) ..controls +(0,0) and +(0.02,.02) .. (.661,-.35);
    \draw[-<-] (.44, .0)  ..controls +(0.2,0.2) and +(0.28,.28) .. (.64,-.3);
    \draw[] (.46, .02)  ..controls +(0,0) and +(0,0) .. (.66,-.285);
\end{scope}

==> sch/ex_comp_plan_3.tex <==
\begin{scope}[yshift=-21,xshift=11.2,rotate=-80,font=\tiny]
    \draw[dotted] (-.23,-.03) circle (.18);
    \node (a) at (-.23,.15) {$*$};
    \draw (-.063,.038)  ..controls +(-0.08,-0.03) and +(-0.01,0.05) .. (-.17,-.201);
    \draw (-.15,-.06) -- (-.4,0.04);
    \draw (-.14,-.04) -- (-.39,0.06);
\end{scope}

==> sch/ex_comp_plan_4.tex <==
\begin{scope}[yshift=10,xshift=12,rotate=100,font=\tiny]
    \draw[dotted] (-.23,-.03) circle (.18);
    \node (a) at (-.23,.15) {$*$};
    \draw (-.063,.038)  ..controls +(-0.08,-0.03) and +(-0.01,0.05) .. (-.17,-.201);
    \draw (-.15,-.06) -- (-.4,0.04);
    \draw (-.14,-.04) -- (-.39,0.06);
\end{scope}

==> sch/ex_comp_plandiag.tex <==
$\ttkz[scale=1.5]{sch/ex_comp_plan_1}: 
\left ( \ttkz[scale=2]{sch/ex_comp_plan_2} , \ttkz[scale=2]{sch/ex_comp_plan_3} ,\ttkz[scale=2]{sch/ex_comp_plan_4} \right )  \mapsto \ttkz[scale=2]{sch/ex_comp_plan}$


==> sch/ex_orange_dot.tex <==
\begin{scope}
  \coordinate (bm) at ( 0, -1);
  \coordinate (cm) at ( 0, -0.6);
  \coordinate (sm) at ( 0,  0.6);
  \coordinate (tm) at ( 0, 1);
  \draw[orange] (-.3,.3) -- (.3,.3) node[pos=.5,below]{$\textcolor{orange}{\omega}$};
  \draw[->] (sm) -- (tm) node[above, pos =1] {};
  \draw[->-] (cm) .. controls + ( 0.6, 0.6) and + ( 0.6, -0.6) .. (sm)
  node [pos = 0.5, right] {} node[pos=.8, draw=orange, fill= white, circle , inner sep=1.5pt]{};
  \draw[->-] (cm) .. controls + (-0.6, 0.6) and + (-0.6, -0.6) .. (sm)
  node [pos = 0.5,  left] {} node[pos=.8, draw=orange, fill= white, circle , inner sep=1.5pt]{};
  \draw[>-] (bm) -- (cm) node[below, pos =0] {};
\end{scope}

==> sch/ex_sliding_2.tex <==
\begin{scope}
    \coordinate (bl) at (-0.5, -1);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (bm) at (  0,-0.3);
    \coordinate (tl) at (-.5,  1);
    \coordinate (tr) at ( 0.5,  1);
    \coordinate (tm) at (  0, 0.3);
    \draw[->, color=blue] (br) -- (tr);
    \draw[->] (bl) -- (tl);
    \draw (-.5, 1) arc (-180:0:-0.5) -- (-1.5,-1) arc (-180:0:0.5);
    \draw[color = blue] (.5, 1) arc (180:0:0.5)  -- (1.5,-1) arc (0:-180:0.5);
\end{scope}

==> sch/ex_sliding_4.tex <==
\begin{scope}
    \coordinate (bl) at (-0.5, -1);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (bm) at (  0,-0.3);
    \coordinate (tl) at (-.5,  1);
    \coordinate (tr) at ( 0.5,  1);
    \coordinate (tm) at (  0, 0.3);
    \draw[->,color=blue] (br) -- (tr);
    \draw[->] (bl) -- (tl);
    \draw (-.5, 1) arc (-180:0:-0.5) -- (-1.5,-1) arc (-180:0:0.5);
    \draw[color=blue] (.5, 1) arc (180:0:0.5) -- (1.5,-1) arc (0:-180:0.5) node[pos=.5, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=.5, above]{$\frac{s}{2}$};
\end{scope}

==> sch/foam_3_local_models.tex <==
\begin{scope}[font =\small]
\tdplotsetmaincoords{80}{140}
  \begin{scope}[tdplot_main_coords]
    \filldraw [very thin, fill=white , fill opacity = 0, draw opacity = 1] (0,-1, -1) -- (0,1,-1) -- (0,1,1) -- (0,-1,1) -- (0,-1,-1);
    \node[sloped, black] at (0,0,0) {$a$};
  \end{scope}
\begin{scope}[xshift = 3cm, tdplot_main_coords]
  \begin{scope}
    \filldraw [very thin, fill =white , fill opacity = 0, draw opacity = 1] (0,-1, -1) -- (0,1,-1) -- (0,1,0) -- (0,-1,0) -- (0,-1,-1);
        \node[sloped, black] at (0,0,-0.5) {$a+b$};
    \end{scope}
  \begin{scope}[rotate around y = 150]
    \filldraw [very thin, fill =white , fill opacity = 0, draw opacity = 1] (0,-1, -1) -- (0,1,-1) -- (0,1,0) -- (0,-1,0) -- (0,-1,-1);
        \node[sloped, black] at (0,0,-0.5) {$a$};
  \end{scope}
  \begin{scope}[rotate around y =-130]
    \filldraw [very thin, fill =white , fill opacity = 0, draw opacity = 1] (0,-1, -1) -- (0,1,-1) -- (0,1,0) -- (0,-1,0) -- (0,-1,-1);
        \node[sloped, black] at (0,0,-0.5) {$b$};
        \draw[very thin, ->-] (0,1,0) -- (0,-1,0);
  \end{scope}
  \end{scope}
\begin{scope}[scale = 1.6, xshift = 4.5cm, tdplot_main_coords]
  \begin{scope}
    \filldraw [very thin, fill =white , fill opacity = 0, draw opacity = 1] (0,-1, -1) -- (0,1,-1) -- (0,1,0) -- (0,0,0) -- (0,-1,-1);
    \coordinate (a) at (0, -1, -1);
        \node[sloped, black] at (0,0.2,-0.5) {$a+b+c$};
    \end{scope}
  \begin{scope}[rotate around y = 150]
    \filldraw [very thin, fill=white , fill opacity = 0, draw opacity = 1] (0,-1, -1) -- (0,1,-1) -- (0,1,0) -- (0,0,0) -- (0,-1,-1);
    \coordinate (b) at (0, -1, -1);
    \node[sloped, black] at (0,0.5,-0.5) {$a+b$};
  \end{scope}
  \begin{scope}[rotate around y =-130]
    \filldraw [very thin, fill=white , fill opacity = 0, draw opacity = 1] (0,-1, -1) -- (0,1,-1) -- (0,1,0) -- (0,0,0) -- (0,-1,-1);
    \coordinate (c) at (0, -1, -1);
        \node[sloped, black] at (0,0.5,-0.5) {$c$};
        \node[sloped, black] at (0,+0.5,-1.5) {$b$};
        \node[sloped, black] at (0,-1.3,0.1) {$b+c$};
        \node[sloped, black] at (0,-0.5,0) {$a$};
  \end{scope}
  \filldraw[very thin, fill=white , fill opacity = 0, draw opacity = 1] (a) -- (b) -- (0,0,0) -- (a);
  \filldraw[very thin, fill=white , fill opacity = 0, draw opacity = 1] (a) -- (c) -- (0,0,0) -- (a);
  \filldraw[very thin, fill=white , fill opacity = 0, draw opacity = 1] (b) -- (c) -- (0,0,0) -- (b);
  \draw[very thin, ->-] (a) -- (0,0,0);
  \draw[very thin, -<-] (b) -- (0,0,0);
  \draw[very thin, ->-] (c) -- (0,0,0);
  \draw[very thin, -<-] (0,1, 0) -- (0,0,0);
\end{scope}
\end{scope}

==> sch/foam_cap_empty.tex <==
\begin{scope}[-]
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm);
  \draw[very thin] (0,0) arc (180 :0: 0.5cm and 0.6cm) node[pos=0.5,
  below] {};
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm)node[ below, pos =0.5] {};
\end{scope}

==> sch/foam_cup_decoN-2.tex <==
\begin{scope}
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) 
  node[above, pos=0.5] {};
  \draw[very thin] (0,0) arc (180 :0: 0.5cm and -0.6cm) node[pos=0.5, above, scale=0.8] {$\deco_{N-2}$};
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm);
\end{scope}

==> sch/foam_cup_deco_n+j.tex <==
\begin{scope}[font=\tiny]
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) node[pos=0.3, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.3,below,yshift=1mm,xshift=2mm]{$-\frac{1}{2}$};
  \draw (0,0) arc (180 :0: 0.5cm and -0.6cm);
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm) node[pos=0.5, below,yshift=-.5mm] {$\deco_{n+i} $};
\end{scope}

==> sch/foam_cup_decorated.tex <==
\begin{scope}[font=\tiny]
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) node[pos=0.3, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.3,below,yshift=1mm,xshift=2mm]{$-\frac{1}{2}$};
  \draw (0,0) arc (180 :0: 0.5cm and -0.6cm);
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm) node[pos=0.5, below,yshift=-.5mm] {$\deco_i $};
\end{scope}


==> sch/foam_cup_decorated_kl.tex <==
\begin{scope}
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) node[pos=0.3, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.3,below,yshift=1mm,xshift=2mm]{$-\frac{1}{2}$};
  \draw (0,0) arc (180 :0: 0.5cm and -0.6cm);
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm) node[pos=0.5, below] {$\deco_{k+i} \antideco_l$};
\end{scope}


==> sch/foam_cup_empty.tex <==
\begin{scope}
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) 
  node[above, pos=0.5] {};
  \draw[very thin] (0,0) arc (180 :0: 0.5cm and -0.6cm) node[pos=0.5, above] {};
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm);
\end{scope}

==> sch/foam_digoncap_01.tex <==
\begin{scope}[font =\tiny]
  \begin{scope}
    \coordinate (L) at (0,0);
    \coordinate (R) at (2,0);
    \coordinate (ML) at (0.5, 0);
    \coordinate (MR) at (1.5, 0);
    \draw[->-] (ML).. controls + (0.4, 0.4) and +(-0.2, 0.4) .. (MR)
    node[above, pos =0.3] {$\deco_0$};    
    \draw[->-] (ML).. controls + (0.2, -0.4) and +(-0.4, -0.4) .. (MR)
    node[above, pos =0.7, yshift = -0.5mm] {$\deco_1$}; %    node[left, pos =0.3] {$1$} 
  \end{scope}  
 \begin{scope}[yshift = 1.3cm]
    \coordinate (LB) at (0,0);
    \coordinate (RB) at (2,0);
    %\draw[double] (LB) -- (RB);
  \end{scope}  
  \draw[double] (MR)--(R) -- (RB) -- (LB) -- (L)-- (ML);
  %\draw[double] (L) -- (LB);
  \draw (ML) .. controls +(0, 1) and +(0, 1) .. (MR);
\end{scope}


==> sch/foam_digoncap_10.tex <==
\begin{scope}[font =\tiny]
  \begin{scope}
    \coordinate (L) at (0,0);
    \coordinate (R) at (2,0);
    \coordinate (ML) at (0.5, 0);
    \coordinate (MR) at (1.5, 0);
    \draw[->-] (ML).. controls + (0.4, 0.4) and +(-0.2, 0.4) .. (MR)
    node[above, pos =0.3] {$\deco_0$}; 
    \draw[->-] (ML).. controls + (0.2, -0.4) and +(-0.4, -0.4) .. (MR)
    node[above, pos =0.7, yshift = -0.5mm] {$\deco_1$}; %    node[left, pos =0.3] {$1$} 
  \end{scope}  
 \begin{scope}[yshift = 1.3cm]
    \coordinate (LB) at (0,0);
    \coordinate (RB) at (2,0);
    %\draw[double] (LB) -- (RB);
  \end{scope}  
  \draw[double] (MR)--(R) -- (RB) -- (LB) -- (L)-- (ML);
  %\draw[double] (L) -- (LB);
  \draw (ML) .. controls +(0, 1) and +(0, 1) .. (MR);
\end{scope}


==> sch/foam_digoncap_empty.tex <==
\begin{scope}[yscale=-1, font=\tiny]
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node
  [pos=0.5, yshift= -0.1cm] {$a$};
  \draw[white!50!black] (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt) node
  [pos=0.5, yshift= 0.1cm, black] {$b$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, below] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}


==> sch/foam_digoncup_01.tex <==
\begin{scope}[font=\tiny]
  \begin{scope}
    \coordinate (L) at (0,0);
    \coordinate (R) at (2,0);
    \coordinate (ML) at (0.5, 0);
    \coordinate (MR) at (1.5, 0);
    \draw[->-] (ML).. controls + (0.4, 0.4) and +(-0.2, 0.4) .. (MR) node[below, pos =0.3] {$\deco_0$};%    node[above, pos=0.7 ] {$1$} 
    \draw[->-] (ML).. controls +(0.2, -0.4) and +(-0.4, -0.4) .. (MR) node[below, pos =0.75] {$\deco_1$};%    node[below, pos =0.3] {$1$} 
  \end{scope}  
 \begin{scope}[yshift = -1.3cm]
    \coordinate (LB) at (0,0);
    \coordinate (RB) at (2,0);

  \end{scope}  
  \draw[double] (MR) -- (R) -- (RB) -- (LB) -- (L) -- (ML);% node[right] {$2$};
  \draw (ML) .. controls +(0, -1) and +(0, -1) .. (MR);
\end{scope}

==> sch/foam_digoncup_0n.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$} node[below, pos =0.6] {$\deco_n$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[below, pos =0.25] {$b$} node[below, pos =0.65] {$\deco_0$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_digoncup_10.tex <==
\begin{scope}[font=\tiny]
  \begin{scope}
    \coordinate (L) at (0,0);
    \coordinate (R) at (2,0);
    \coordinate (ML) at (0.5, 0);
    \coordinate (MR) at (1.5, 0);
    \draw[->-] (ML).. controls + (0.4, 0.4) and +(-0.2, 0.4) .. (MR) node[below, pos =0.3] {$\deco_0$};
    \draw[->-] (ML).. controls +(0.2, -0.4) and +(-0.4, -0.4) .. (MR) node[below, pos =0.75] {$\deco_1$};
  \end{scope}  
 \begin{scope}[yshift = -1.3cm]
    \coordinate (LB) at (0,0);
    \coordinate (RB) at (2,0);
  \end{scope}  
  \draw[double] (MR) -- (R) -- (RB) -- (LB) -- (L) -- (ML);
  \draw (ML) .. controls +(0, -1) and +(0, -1) .. (MR);
\end{scope}

==> sch/foam_digoncup_N.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$} node[below, pos =0.6] {$\deco_n$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[below, pos =0.25] {$b$} ;
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_digoncup_abkl.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[below, pos =0.25] {$b$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} node[below, pos =0.5] {$\deco_l$} -- (Rb) -- (Lb) -- (Lt) -- (lt) node[below, pos =0.5] {$\deco_k$};
\end{scope}

==> sch/foam_digoncup_akl.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$} node[below, pos =0.5] {$\deco_k \deco_l$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[below, pos =0.25] {$b$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_digoncup_bkl.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[above, pos =0.5] {$b$} node[below, pos =0.5,yshift=.25mm] {$\deco_k\deco_l$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_digoncup_empty.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node
  [pos=0.5, yshift= 0.1cm] {$a$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt) node
  [pos=0.5, yshift= -0.1cm] {$b$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_digoncup_kl.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$} node[below, pos =0.6] {$\deco_k$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[below, pos =0.25] {$b$} node[below, pos =0.65] {$\deco_l$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_digoncup_n.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[below, pos =0.25] {$b$} node[below, pos =0.65] {$\deco_n$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_digoncup_n0.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (Lt) at (0,2);
    \coordinate (Rt) at (2,2);
    \coordinate (lt) at (0.5,2);
    \coordinate (rt) at (1.5,2);
    \coordinate (Lb) at (0,1);
    \coordinate (Rb) at (2,1);
  \end{scope}
  \draw (lt) .. controls +(0.3, 0.3) and +(-.3, 0.3) ..  (rt) node[above, pos=0.3] {$a$} node[below, pos =0.6] {$\deco_0$};
  \draw (lt) .. controls +(0.3, -.3) and +(-.3, -.3) ..  (rt)node[below, pos =0.25] {$b$} node[below, pos =0.65] {$\deco_n$};
  \draw (lt) .. controls +(0 , -.9) and +(0, -.9) ..  (rt);
  \draw (rt) -- (Rt) node[pos=1, above] {$a+b$} -- (Rb) -- (Lb) -- (Lt) -- (lt);
\end{scope}

==> sch/foam_sing_saddle_empty.tex <==
\begin{scope}[yscale=0.5, xscale=0.5, font=\tiny]
  \begin{scope}
    \coordinate (At) at (0,0);
    \coordinate (Bt) at (0.5,1);
    \coordinate (Ct) at (3,1);
    \coordinate (Dt) at (2.5,0);
    \coordinate (Et) at (2,0.1);
    \coordinate (Ft) at (1,0.9);
  \end{scope}
  \coordinate (O) at (1.5, -0.5);
  \begin{scope}[yshift= -2cm]
    \coordinate (Ab) at (0,0);
    \coordinate (Bb) at (0.5,1);
    \coordinate (Cb) at (3,1);
    \coordinate (Db) at (2.5,0);
    \coordinate (Eb) at (0.8,0.5);
    \coordinate (Fb) at (2.2,0.5);
  \end{scope}

  \draw (Bt) -- (Bb) -- (Eb) -- (Fb) node[pos=0.5, below] {$a+b+c$}-- (Cb) -- (Ct) -- (Ft) -- (O);
  \filldraw[draw =  black, fill = white, fill opacity=0.5] (At) --
  (Et) -- (Dt) -- (Db) -- (Fb) -- (O) -- (Eb) -- (Ab) -- (At);
  \draw (Bt) -- (Ft)-- (Et) node[pos=0.5, xshift =0.2cm] {$c$} -- (O);

  \begin{scope}
    \node[yshift = -0.15cm] at (Ab) {$b+c$};
    \node[yshift = 0.15cm] at (Bt) {$a$};
    \node[yshift = 0.15cm] at (Ct) {$a+c$};
    \node[yshift = -0.15cm] at (Db) {$b$};
    
  \end{scope}

\end{scope}

==> sch/foam_sing_saddle_empty_2.tex <==
\begin{scope}[yscale=0.5, xscale=0.5, font=\tiny]
  \begin{scope}
    \coordinate (At) at (0,0);
    \coordinate (Bt) at (0.5,1);
    \coordinate (Ct) at (3,1);
    \coordinate (Dt) at (2.5,0);
    \coordinate (Et) at (2,0.1);
    \coordinate (Ft) at (1,0.9);
  \end{scope}
  \coordinate (O) at (1.5, -0.5);
  \begin{scope}[yshift= -2cm]
    \coordinate (Ab) at (0,0);
    \coordinate (Bb) at (0.5,1);
    \coordinate (Cb) at (3,1);
    \coordinate (Db) at (2.5,0);
    \coordinate (Eb) at (0.8,0.5);
    \coordinate (Fb) at (2.2,0.5);
  \end{scope}

  \draw (Bt) -- (Bb) -- (Eb) -- (Fb) node[pos=0.5, below] {$a+b+c$}-- (Cb) -- (Ct) -- (Ft) -- (O);
  \filldraw[draw =  black, fill = white, fill opacity=0.5] (At) --
  (Et) -- (Dt) -- (Db) -- (Fb) -- (O) -- (Eb) -- (Ab) -- (At);
  \draw (Bt) -- (Ft)-- (Et) node[pos=0.5, xshift =0.2cm] {$c$} -- (O);

  \begin{scope}
    \node[xshift = -0.35cm] at (Ab) {$b+c$};
    \node[xshift = -0.2cm] at (Bt) {$a$};
    \node[xshift = 0.35cm] at (Ct) {$a+c$};
    \node[xshift = 0.15cm] at (Db) {$b$};
    
  \end{scope}

\end{scope}

==> sch/hopflink_2.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5) .. controls +(0,-0.5) and +(0, 0.5) .. (0.5, -0.5);
	\fill[white] (0, 0) circle (1mm);
	\draw[-] (-0.5, -0.5) .. controls +(0,0.5) and +(0, -0.5) .. (0.5, 0.5);

	\draw (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,-0.5) arc (-180:0:0.5)  ;
	\draw (0.5, 2) arc (180:0:0.5)  -- (1.5,-0.5) arc (0:-180:0.5)  ;

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s$};
\end{scope}


==> sch/hopflink_3.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw[-] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5);
	\fill[white] (0,0) circle (2mm);
	\draw[-] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5,0.5);

	\draw (-0.5, 0.5) arc (-180:0:-0.5)  -- (-1.5,-0.5) arc (-180:0:0.5)  ;
	\draw (0.5, 0.5) arc (180:0:0.5)  -- (1.5,-0.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/hopflink_4.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,0.5) arc (-180:0:0.5)  ;
	\draw (0.5, 2) arc (180:0:0.5)  -- (1.5,0.5) arc (0:-180:0.5)  ;

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5);
	\draw[-] (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1, yshift=1mm,right]{$s+1$};
\end{scope}


==> sch/hopflink_5.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,0.5) arc (-180:0:0.5)  -- (-0.5,2)
	      node[draw=\crd, fill=\csrd, circle, inner sep=1.5pt, pos=0]{} node[pos=0, right]{$-\frac{1}{2}$};
\end{scope}


==> sch/identity_X.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (L1) at (0.2,0.4);
    \coordinate (L2) at (0,0);
    \coordinate (R1) at (2.2,0.4);
    \coordinate (R2) at (2,0);
    \coordinate (ML) at (0.6, 0.2);
    \coordinate (MR) at (1.6, 0.2);
    \draw[double] (ML) -- (MR) node[above, midway] {};
    \draw (MR) .. controls +(0, 0) and +(-0.3,0) .. (R1);
    \draw (MR) .. controls +(0, 0) and +(-0.3,0) .. (R2);
    \draw (L1) .. controls +( 0.3, 0) and +(0,0) .. (ML);
    \draw (L2) .. controls +( 0.3, 0) and +(0,0) .. (ML);
    \draw[dotted] (L2) ..controls +(-.8,-.8) and +(.6,-.6) .. (R2);
    \draw[dotted] (L1) ..controls +(-.4,.4) and +(.6,.6) .. (R1);
  \end{scope}  
 \begin{scope}[yshift = -1cm]
    \coordinate (L1B) at (0.2,0.4);
    \coordinate (L2B) at (0,0);
    \coordinate (R1B) at (2.2,0.4);
    \coordinate (R2B) at (2,0);
    \coordinate (MLB) at (0.6, 0.2);
    \coordinate (MRB) at (1.6, 0.2);
    \coordinate (R3B) at (2.2,.5);
    \draw[double] (MLB) -- (MRB) node[above, midway] {};
    \draw (MRB) .. controls +(0, 0) and +(-0.3,0) .. (R1B) ;
    \draw (MRB) .. controls +(0, 0) and +(-0.3,0) .. (R2B) node[above, pos =0.8] {$\deco_1$};
    \draw (L1B) .. controls +( 0.3, 0) and +(0,0) .. (MLB);
    \draw (L2B) .. controls +( 0.3, 0) and +(0,0) .. (MLB);
    \draw[dotted] (L2B) ..controls +(-.8,-.8) and +(.6,-.6) .. (R2B);
    \draw[dotted] (R1B) ..controls +(.1,.1) and +(.1,.1) .. (R3B);
 \end{scope}  
  \draw (R1) -- (R1B);
  \draw (R2) -- (R2B);
  \draw (L1) -- (L1B);
  \draw (L2) -- (L2B);
  \draw (ML) -- (MLB);
  \draw (MR) -- (MRB);
\end{scope}

==> sch/identity_X_1.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (L1) at (0.2,0.4);
    \coordinate (L2) at (0,0);
    \coordinate (R1) at (2.2,0.4);
    \coordinate (R2) at (2,0);
    \coordinate (ML) at (0.6, 0.2);
    \coordinate (MR) at (1.6, 0.2);
    \draw[double] (ML) -- (MR) node[above, midway] {};
    \draw (MR) .. controls +(0, 0) and +(-0.3,0) .. (R1);
    \draw (MR) .. controls +(0, 0) and +(-0.3,0) .. (R2);
    \draw (L1) .. controls +( 0.3, 0) and +(0,0) .. (ML);
    \draw (L2) .. controls +( 0.3, 0) and +(0,0) .. (ML);
    \draw[dotted] (L2) ..controls +(-.8,-.8) and +(.6,-.6) .. (R2);
    \draw[dotted] (L1) ..controls +(-.4,.4) and +(.6,.6) .. (R1);
  \end{scope}  
 \begin{scope}[yshift = -1cm]
    \coordinate (L1B) at (0.2,0.4);
    \coordinate (L2B) at (0,0);
    \coordinate (R1B) at (2.2,0.4);
    \coordinate (R2B) at (2,0);
    \coordinate (MLB) at (0.6, 0.2);
    \coordinate (MRB) at (1.6, 0.2);
    \coordinate (R3B) at (2.2,.5);
    \draw[double] (MLB) -- (MRB) node[above, midway] {};
    \draw (MRB) .. controls +(0, 0) and +(-0.3,0) .. (R1B) ;
    \draw (MRB) .. controls +(0, 0) and +(-0.3,0) .. (R2B);
    \draw (L1B) .. controls +( 0.3, 0) and +(0,0) .. (MLB);
    \draw (L2B) .. controls +( 0.3, 0) and +(0,0) .. (MLB) node[above, pos =0.2] {$\deco_1$};
    \draw[dotted] (L2B) ..controls +(-.8,-.8) and +(.6,-.6) .. (R2B);
    \draw[dotted] (R1B) ..controls +(.1,.1) and +(.1,.1) .. (R3B);
 \end{scope}  
  \draw (R1) -- (R1B);
  \draw (R2) -- (R2B);
  \draw (L1) -- (L1B);
  \draw (L2) -- (L2B);
  \draw (ML) -- (MLB);
  \draw (MR) -- (MRB);
\end{scope}

==> sch/identity_Y.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (L1) at (0.2,0.4);
    \coordinate (L2) at (0,0);
    \coordinate (R1) at (2.2,0.4);
    \coordinate (R2) at (2,0);
    \coordinate (ML) at (0.6, 0.2);
    \coordinate (MR) at (1.6, 0.2);
    
    \draw[double] (ML) -- (MR) node[above, midway] {};
    \draw (MR) .. controls +(0, 0) and +(-0.3,0) .. (R1);
    \draw (MR) .. controls +(0, 0) and +(-0.3,0) .. (R2);
    \draw (L1) .. controls +( 0.3, 0) and +(0,0) .. (ML) node[below, pos =0.3] {$\deco_1$};
    \draw (L2) .. controls +( 0.3, 0) and +(0,0) .. (ML);
    \draw[dotted] (L2) ..controls +(-.8,-.8) and +(.6,-.6) .. (R2);
    \draw[dotted] (L1) ..controls +(-.4,.4) and +(.6,.6) .. (R1);
  \end{scope}  
 \begin{scope}[yshift = -1cm]
    \coordinate (L1B) at (0.2,0.4);
    \coordinate (L2B) at (0,0);
    \coordinate (R1B) at (2.2,0.4);
    \coordinate (R2B) at (2,0);
    \coordinate (MLB) at (0.6, 0.2);
    \coordinate (MRB) at (1.6, 0.2);
    \coordinate (R3B) at (2.2,.5);
    \draw[double] (MLB) -- (MRB) node[above, midway] {};
    \draw (MRB) .. controls +(0, 0) and +(-0.3,0) .. (R1B) ;
    \draw (MRB) .. controls +(0, 0) and +(-0.3,0) .. (R2B);
    \draw (L1B) .. controls +( 0.3, 0) and +(0,0) .. (MLB);
    \draw (L2B) .. controls +( 0.3, 0) and +(0,0) .. (MLB);
    \draw[dotted] (L2B) ..controls +(-.8,-.8) and +(.6,-.6) .. (R2B);
    \draw[dotted] (R1B) ..controls +(.1,.1) and +(.1,.1) .. (R3B);
 \end{scope}  
  \draw (R1) -- (R1B);
  \draw (R2) -- (R2B);
  \draw (L1) -- (L1B);
  \draw (L2) -- (L2B);
  \draw (ML) -- (MLB);
  \draw (MR) -- (MRB);
\end{scope}

==> sch/meteorite_1.tex <==
\begin{scope}[font=\tiny]
    \draw[dotted] (0,0) circle (.5);
    \draw[fill=black] (0,0) circle (.05);
\end{scope}

==> sch/movie_r2b_1.tex <==
\begin{scope}
    \coordinate (a) at (0.6, -0.3);
    \coordinate (b) at (0.6, 1.3);
    \draw [<-](0, 0) .. controls +(1,.5).. (2, 0);
    \draw [->](0, 1) .. controls +(1,-.5).. (2, 1);
    \draw [-<] (a) arc (180:0:0.4);
    \draw [-] (a) arc (-180:0:0.4);
    \draw [-<] (b) arc (180:0:0.4);
    \draw [-] (b) arc (-180:0:0.4);
\end{scope}


==> sch/movie_r2b_3.tex <==
\begin{scope}
    \coordinate (bl) at (-0.5, -1.5);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (tr) at ( 0.5,  1);
    \coordinate (tl) at (-0.5,  1.5);
    \coordinate (bm) at (  0,-0.4);
    \coordinate (tm) at (  0, 0.4);
    \coordinate (bl2) at (1.5, -1);
    \coordinate (br2) at ( 2.5, -1.5);
    \coordinate (bm2) at (  2,-0.4);
    \coordinate (tl2) at (1.5,  1);
    \coordinate (tr2) at ( 2.5,  1.5);
    \coordinate (tm2) at ( 2, 0.4);
    \draw[<-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm);
    \draw[<-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
    \draw[>-]  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm) coordinate[pos = 0.25] (ga) ;
    \draw[>-]  (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm) coordinate[pos = 0.25] (gb) ;
    \draw [double] (bm) -- (tm);
    \draw (.5, 1) arc (180:0:0.5);
    \draw (1.5,-1) arc (180:0:-0.5);
    \draw[>-]  (bl2) .. controls +( 0, 0.5) and +(0,0) .. (bm2);
    \draw[>-]  (br2) .. controls +( 0, 0.5) and +(0,0) .. (bm2);
    \draw[<-]  (tl2) .. controls +( 0, -0.5) and +(0,0) .. (tm2);
    \draw [double] (bm2) -- (tm2);
    \draw[<-]  (tr2) .. controls +( 0, -0.5) and +(0,0) .. (tm2); 
\end{scope}

==> sch/movie_r3_1.tex <==
\begin{scope}
    \coordinate (au) at (-.5,1.3);
    \coordinate (bu) at (.5,1.3);
    \coordinate (cu) at (1.5,1.3); 
    \coordinate (abu) at (0,0.5);
    \coordinate (abcu) at (.5,0);
    \draw[<-] (au) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[<-]  (bu) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[double] (abu) .. controls +( 0, -0.5) and +(0,0) .. (abcu); 
    \draw[<-] (cu) .. controls +( 0, -0.7) and +(0,0) .. (abcu);
    \coordinate (ad) at (-.5,-2.3);
    \coordinate (bd) at (.5,-2.3);
    \coordinate (cd) at (1.5,-2.3); 
    \coordinate (abd) at (0,-1.5);
    \coordinate (abcd) at (.5,-1);
    \draw[>-] (ad) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[>-]  (bd) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[double] (abd) .. controls +( 0,0.5) and +(0,0) .. (abcd); 
    \draw[>-] (cd) .. controls +( 0,0.7) and +(0,0) .. (abcd);
    \draw[line width=.7mm] (abcd) -- (abcu) coordinate[pos = 0.5] (ga);
\end{scope}

==> sch/movie_r3_2.tex <==
\begin{scope}
    \coordinate (au) at (-.5,1.3);
    \coordinate (bu) at (.5,1.3);
    \coordinate (cu) at (1.5,1.3); 
    \coordinate (abu) at (0,0.7);
    \coordinate (abup) at (0.07,.5);
    \coordinate (abupp) at (0.25,.2);
    \coordinate (abcu) at (.5,0);
    \draw[<-] (au) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[<-]  (bu) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[double] (abu) .. controls +( 0, -0.1) and +(0,0) .. (abup); 
    \draw[double] (abupp) .. controls +( 0,0) and +(0,-0.1) .. (abcu); 
    \draw[] (abup) .. controls +(0.4,0.08) and +(0,0) .. (abupp);
    \draw[] (abup) .. controls +(-.2,-0.4) and +(0,0) .. (abupp);
    \draw[<-] (cu) .. controls +( 0, -0.7) and +(0,0) .. (abcu);
    \coordinate (ad) at (-.5,-2.3);
    \coordinate (bd) at (.5,-2.3);
    \coordinate (cd) at (1.5,-2.3); 
    \coordinate (abd) at (0,-1.5);
    \coordinate (abcd) at (.5,-1);
    \draw[>-] (ad) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[>-]  (bd) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[double] (abd) .. controls +( 0,0.5) and +(0,0) .. (abcd); 
    \draw[>-] (cd) .. controls +( 0,0.7) and +(0,0) .. (abcd);
    \draw[line width=.7mm] (abcd) -- (abcu) coordinate[pos = 0.5] (ga);
\end{scope}

==> sch/movie_r3_3.tex <==
\begin{scope}
    \coordinate (au) at (-.5,1.3);
    \coordinate (bu) at (.5,1.3);
    \coordinate (cu) at (1.5,1.3); 
    \coordinate (abu) at (0,0.7);
    \coordinate (abup) at (0.07,.5);
    \coordinate (bcu) at (0.95,.3);
    \coordinate (abcu) at (.5,-.1);
    \draw[<-] (au) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[<-]  (bu) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[-<-] (abup) .. controls +(0.4,0.08) and +(0,0) .. (bcu);
    \draw[-<-] (abup) .. controls +(-.15,-0.6) and +(0,0) .. (abcu);
    \draw[<-] (cu) .. controls +( 0, -0.7) and +(0,0) .. (bcu);
    \draw[double] (abu) .. controls +( 0, -0.1) and +(0,0) .. (abup); 
    \draw[double] (bcu) .. controls +(-0.1,-0.3) and +(0,0) .. (abcu); 
    \coordinate (ad) at (-.5,-2.3);
    \coordinate (bd) at (.5,-2.3);
    \coordinate (cd) at (1.5,-2.3); 
    \coordinate (abd) at (0,-1.5);
    \coordinate (abcd) at (.5,-1);
    \draw[>-] (ad) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[>-]  (bd) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[double] (abd) .. controls +( 0,0.5) and +(0,0) .. (abcd); 
    \draw[>-] (cd) .. controls +( 0,0.7) and +(0,0) .. (abcd);
    \draw[line width=.7mm] (abcd) -- (abcu) coordinate[pos = 0.5] (ga);
\end{scope}

==> sch/movie_r3_4.tex <==
 \begin{scope}
    \coordinate (au) at (-.5,1.3);
    \coordinate (bu) at (.5,1.3);
    \coordinate (cu) at (1.5,1.3); 
    \coordinate (abu) at (0,0.6);
    \coordinate (abup) at (0,.15);
    \coordinate (bcu) at (0.95,-.1);
    \coordinate (abcu) at (.95,-.7);
    \draw[<-] (au) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[<-]  (bu) .. controls +( 0, -0.5) and +(0,0) .. (abu);
    \draw[-<-] (abup) -- (bcu);
    \draw[<-] (cu) .. controls +( 0, -0.7) and +(0,0) .. (bcu);
    \draw[double] (abu) .. controls +( 0, -0.1) and +(0,0) .. (abup); 
    \draw[double] (bcu) .. controls +(0,0) and +(0,0) .. (abcu); 
    \coordinate (ad) at (-.5,-2.3);
    \coordinate (bd) at (.5,-2.3);
    \coordinate (cd) at (1.5,-2.3); 
    \coordinate (abd) at (0,-1.5);
    \coordinate (abcd) at (0,-1);
    \draw[>-] (ad) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[>-]  (bd) .. controls +( 0,0.5) and +(0,0) .. (abd);
    \draw[double] (abd) .. controls +( 0,0.5) and +(0,0) .. (abcd); 
    \draw[>-] (cd) .. controls +( 0,0.7) and +(0,0) .. (abcu);
    \draw[->-] (abcd) -- (abcu);
    \draw[-<-] (abup) -- (abcd);
\end{scope}

==> sch/notation_antideco.tex <==
\begin{scope}
    \draw (-1,-1) rectangle (1,1) coordinate [midway] (A);
  \fill (A) circle (0.5mm) node[below] {$\widehat{p}_i$};
\end{scope}

==> sch/notation_deco1.tex <==
\begin{scope}
  \draw (-1,-1) rectangle (1,1) coordinate [midway] (A);
  \fill (A) circle (0.5mm) node[below] {$p_i$};
\end{scope}

==> sch/notation_deco2.tex <==
\begin{scope}
  \draw (-1,-1) rectangle (1,1);
  \coordinate (.5,.5) node[]{$\deco_i$};
\end{scope}

==> sch/notation_deco3.tex <==
\begin{scope}
  \draw (-1,-1) rectangle (1,1);
  \coordinate (.5,.5) node[]{$\antideco_i$};
\end{scope}

==> sch/red_dot_circular_hollow.tex <==
\begin{scope}
    \node(A) at (0,0) [draw=\crd, fill= white, circle , inner sep=2pt]{};
\end{scope}

==> sch/red_dot_circular_solid.tex <==
\begin{scope}
    \node(A) at (0,0) [draw=\crd, fill= \csrd, circle , inner sep=2pt]{};
\end{scope}

==> sch/red_dot_double_orange.tex <==
\begin{scope}
    \node(A) at (0,0) [draw=orange, fill= white, circle , inner sep=2pt]{};
    \node(B) at (.4,0) [draw=orange, fill= white, circle , inner sep=2pt]{};
    \draw[orange] (A)--(B);
\end{scope}

==> sch/red_dot_triangle.tex <==
\begin{scope}
    \node(A) at (0,0) [draw=\crd, fill=white, regular polygon, regular polygon sides=3,inner sep=1.2pt] {};
\end{scope}

==> sch/reidem1_6.tex <==
\begin{scope}
  \draw [->] (0, -1) -- +(0,2);
   \coordinate (O) at (1, 0);
       \filldraw[draw= \crd, fill = \csrd] (O);
     \coordinate (A) at (0, -.6);
        \filldraw[draw= \crd, fill = white] (A);
\end{scope}

==> sch/reidem1_7.tex <==
\begin{scope}
    \coordinate (bl) at (-0.5, -1);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (tl) at (-0.5,  1);
    \coordinate (tr) at ( 0.5,  1);
    \coordinate (Oo) at (2.5,0);
    \coordinate (ml) at (-0.5,  -.8);
    \coordinate (Ml) at (-0.5,  .8);
    \coordinate (mr) at (0.5,  -.6);
    \coordinate (Mr) at (0.5,  .6);
    \draw[->] (bl) -- (tl);  
    \draw[->] (br) -- (tr);
    \draw (.5, 1) arc (180:0:0.5) -- (1.5,-1) arc (180:0:-0.5);
    \coordinate (A) at (1.5, -.8);
    \filldraw[draw= \crd, fill = \csrd] (A) circle (1mm) node[right] {$-\frac{1}{2}$};
    \coordinate (B) at (1.5, .8);
\end{scope}

==> sch/reidem1_8.tex <==

\begin{scope}
  \coordinate (bl) at (-0.5, -1);
  \coordinate (br) at ( 0.5, -1);
  \coordinate (bm) at (  0,-0.3);
  \coordinate (tl) at (-0.5,  1);
  \coordinate (tr) at ( 0.5,  1);
  \coordinate (tm) at (  0, 0.3);
  \draw[>-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[>-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[<-]  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm) coordinate[pos = 0.25] node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node [pos=0.3, left]{$\lambda$};
  \draw[<-]  (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm)
  coordinate[pos = 0.25] node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
  \draw [double] (bm) -- (tm) node[pos=0, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=0, right]{$-\bar{s}$};
  \draw (.5, 1) arc (180:0:0.5) -- (1.5,-.85) arc (180:0:-0.5);
    \coordinate (A) at (1.5, -.8);
    \coordinate (B) at (1.5, .8);
    \filldraw[draw= \crd, fill = \csrd] (A) circle (1mm)
    node[right] {$-\frac{1}{2}$};
    \coordinate (Oo) at (2.7,0);
\end{scope}


==> sch/reidem2a_1.tex <==
\begin{scope}
  \coordinate (bl) at (-0.5, -1);
  \coordinate (br) at ( 0.5, -1);
  \coordinate (bm) at (  0,-0.3);
  \coordinate (tl) at (-0.5,  1);
  \coordinate (tr) at ( 0.5,  1);
  \coordinate (tm) at (  0, 0.3);
  \draw[>-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[>-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[<-]  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw[<-]  (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw [double] (bm) -- (tm);
\end{scope}

==> sch/reidem2a_2.tex <==
\begin{scope}
    \coordinate (bl) at (-0.5, -1);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (bm) at (  0,-0.3);
    \coordinate (tl) at (-0.5,  1);
    \coordinate (tr) at ( 0.5,  1);
    \coordinate (tm) at (  0, 0.3);
    \coordinate (brr) at ( 1.5, -1);
    \coordinate (trr) at ( 1.5, 1);
    \draw[>-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm) ;
    \draw[>-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
    \draw[<-]  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm);
    \draw[<-]  (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm);
    \draw [double] (bm) -- (tm) node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1, right, yshift=-.5mm]{$s$}; 
    \coordinate (blU) at (-0.5, 1);
    \coordinate (brU) at ( 0.5, 1);
    \coordinate (bmU) at (  0,1.7);
    \coordinate (tlU) at (-0.5,  3);
    \coordinate (trU) at ( 0.5,  3);
    \coordinate (tmU) at (  0, 2.3);
    \coordinate (brrU) at ( 1.5, 1);
    \coordinate (trrU) at ( 1.5, 3);
    \draw[]  (blU) .. controls +( 0, 0.5) and +(0,0) .. (bmU) node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
    \draw[]  (brU) .. controls +( 0, 0.5) and +(0,0) .. (bmU) node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
    \draw[<-]  (tlU) .. controls +( 0, -0.5) and +(0,0) .. (tmU) coordinate[pos = 0.25] (gaU) ;
    \draw[<-]  (trU) .. controls +( 0, -0.5) and +(0,0) .. (tmU) coordinate[pos = 0.25] (gbU) ;  
    \draw [double] (bmU) -- (tmU);
\end{scope}

==> sch/reidem2a_3.tex <==
\begin{scope}
  \coordinate (bl) at (-0.5, -1);
  \coordinate (br) at ( 0.5, -1);
  \coordinate (bm) at (  0,-0.3);
  \coordinate (tl) at (-0.5,  1);
  \coordinate (tr) at ( 0.5,  1);
  \coordinate (tm) at (  0, 0.3);
  \draw[>-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[>-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[<-]  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw[<-]  (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw [double] (bm) -- (tm) node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1, right, yshift=-.5mm]{$1$};
\end{scope}

==> sch/reidem2b_2p.tex <==
\begin{scope}[xshift = 2.5cm]
  \draw [<-] (0, -0.5) .. controls +(.5,0) and +(-.5, 0)
  .. (1, 0.5)  ; 
    \fill[white] (0.5, 0) circle (1mm);
    \draw(0, 0.5) .. controls +(.5,0) and +(-.5, 0)
  .. (1, -0.5) ;
  \draw[] (1, 0.5) .. controls +(.5,0) and +(-.5, 0)
  .. (2, -0.5)  node[pos=0.25, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.25, left, yshift=-2.5mm]{$\frac{1}{2}$}
  node[pos=0.7, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.7, above, xshift=2mm, yshift=-1mm]{$-\frac{1}{2}$};
    \fill[white] (1.5, 0) circle (1mm);  
      \draw[<-] (2, 0.5)  .. controls +(-.5,0) and +(.5, 0)
  .. (1, -0.5); 
\end{scope}

==> sch/reidem2b_4.tex <==
\begin{scope}
    \coordinate (bl) at (0, -1);
    \coordinate (br) at (2, -1);
    \coordinate (tl) at (0,  1);
    \coordinate (tr) at (2,  1);
    \coordinate (ml) at (-0.5,  -.8);
    \coordinate (Ml) at (-0.5,  .8);
    \coordinate (mr) at (0.5,  -.6);
    \coordinate (Mr) at (0.5,  .6);
    \draw[<-<] (bl) -- (tl);
    \draw[>->] (br) -- (tr) node[pos=0.5, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.5, right]{$-\frac{1}{2}$};
    \draw [-<] (.5, 0) arc (180:0:0.5) node[pos=0.5, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.5, above]{$\frac{1}{2}$};
    \draw (.5, 0) arc (-180:0:0.5) ;
\end{scope}

==> sch/reidem2b_8.tex <==
\begin{scope}
  \coordinate (m) at (  0,  0);
  \coordinate (t) at (  0, 0.75);
  \coordinate (br) at (+.5,  -.8);
  \coordinate (bl) at (-.5,  -.8);
  \draw[<-] (bl) .. controls +(0,0.5) and + (0, 0) .. (m) node[pos=0.3, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.3, left]{$\frac{1}{2}$};
  \draw[<-] (br) .. controls +(0,0.5) and + (0, 0) .. (m) node[pos=0.3]{} ;
  \draw[double] (m) -- (t) node[pos=0.7, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.7, right]{$-\frac{1}{2}$} 
  node[pos=0, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=0, right]{$-\bar{s}$};
\end{scope}

==> sch/reidem3_2.tex <==
\begin{scope}
    \coordinate (bl) at (-0.5, -1);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (tl) at (-0.5,  1);
    \coordinate (tr) at ( 0.5,  1);
    \coordinate (ml) at (-0.5,  -.8);
    \coordinate (Ml) at (-0.5,  .8);
    \coordinate (mr) at (0.5,  -.6);
    \coordinate (Mr) at (0.5,  .6);
    \coordinate (brr) at ( 1.5, -1);
    \coordinate (trr) at ( 1.5, 1);
    \draw[->-] (bl) -- (tl);
    \draw[->-] (br) -- (tr); 
    \draw[->-] (brr) -- (trr);
\end{scope}

==> sch/reidem_lemm_10.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5,0.5) node[pos=1, above] {};
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=0.75, draw=\crd, fill= white, circle , inner sep=2pt]{} node[pos=0.75, right]{$\omega$};
\end{scope}

==> sch/reidem_lemm_19.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t1) ;
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t2);
  \filldraw[draw= \crd, fill = white] (t2) circle (1mm)
  node[left] {$\omega$};
  \filldraw[draw= \crd, fill = white] (t1) circle (1mm)
  node[right] {$\omega$};
\end{scope}

==> sch/reidem_lemm_20.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5,0.5) node[pos=1, above] {} coordinate[pos =0.75] (t1);
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.75] (t2);
  \filldraw[draw= \crd, fill = white] (t2) circle (1mm)
  node[right] {$\omega$};
  \filldraw[draw= \crd, fill = white] (t1) circle (1mm)
  node[left] {$\omega$};
\end{scope}

==> sch/reidem_lemm_23.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t1) ;
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.15] (t2) coordinate[pos=0.35] (t3);
  \filldraw[draw= \crd, fill = white] (t1) circle (1mm)
  node[right] {$\epsilon$};
  \filldraw[draw= \crd, fill = white] (t2) circle (1mm)
  node[left] {$\epsilon$};
  \filldraw[draw= \crd, fill = white] (t3) circle (1mm)
  node[left] {$\omega-\epsilon$};
\end{scope}

==> sch/reidem_lemm_24.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t1) ;
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t2) coordinate[pos=0.7] (t3);
  \filldraw[draw= \crd, fill = white] (t1) circle (1mm)
  node[right] {$\epsilon$};
  \filldraw[draw= \crd, fill = white] (t2) circle (1mm)
  node[left] {$\epsilon$};
  \filldraw[draw= \crd, fill = white] (t3) circle (1mm)
  node[right] {$\omega-\epsilon$};
\end{scope}

==> sch/reidem_lemm_27.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t1);
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t2);
  \filldraw[draw= \crd, fill = \csrd] (t2) circle (1mm)
  node[left] {$\omega$};
\end{scope}

==> sch/reidem_lemm_28.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5,0.5) node[pos=1, above] {} coordinate[pos =0.75] (t1);
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.75] (t2);
  \filldraw[draw= \crd, fill = \csrd] (t2) circle (1mm)
  node[right] {$\omega$};
\end{scope}

==> sch/reidem_lemm_29.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t1);
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.2] (t2);
  \filldraw[draw=black, fill = black] (t2) circle (1mm)
  node[left] {$\omega$};
\end{scope}

==> sch/reidem_lemm_30.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5,0.5) node[pos=1, above] {} coordinate[pos =0.75] (t1);
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=1, above] {} coordinate[pos =0.75] (t2);
  \filldraw[draw=black, fill = black] (t2) circle (1mm)
  node[right] {$\omega$};
\end{scope}

==> sch/reidem_lemm_9.tex <==
\begin{scope}[font=\tiny]
  \draw[->] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5) node[pos=1, above] {};
  \fill[white] (0,0) circle (2mm);
  \draw[->] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5, 0.5) node[pos=0.2, draw=\crd, fill= white, circle , inner sep=2pt]{} node[pos=0.2, left]{$\omega$};
\end{scope}

==> sch/relation_add_dots1.tex <==
\begin{scope}
  \coordinate (m) at (0,0);
  \coordinate (t) at (2,0);
  \draw[->] (m) -- (t) node[pos = 1, right] {$a$} coordinate[pos=0.3] (ga) coordinate[pos=0.7] (gb);
  \filldraw[draw= \crd, fill = white] (ga) circle (1mm) node[yshift= 3mm] {\color{\crd}$\omega_1$};
  \filldraw[draw= \crd, fill = white] (gb) circle (1mm) node[yshift=3mm] {\color{\crd}$\omega_2$};
\end{scope}

==> sch/relation_add_dots2.tex <==
\begin{scope}
  \coordinate (m) at (0,0);
  \coordinate (t) at (2,0);
  \draw[->] (m) -- (t) node[pos = 1, right] {$a$} coordinate[pos=0.5] (ga) coordinate[pos=0.7] (gb);
  \filldraw[draw= \crd, fill = white] (ga) circle (1mm) node[yshift= 3mm] {\color{\crd}$\omega_1+\omega_2$};
\end{scope}

==> sch/relation_add_dots3.tex <==
\begin{scope}
  \coordinate (m) at (0,0);
  \coordinate (t) at (2,0);
  \draw[->] (m) -- (t) node[pos = 1, right] {$a$} coordinate[pos=0.3] (ga) coordinate[pos=0.7] (gb);
  \filldraw[draw= \crd, fill = \csrd] (ga) circle (1mm) node[yshift= 3mm] {\color{\crd}$\omega_1$};
  \filldraw[draw= \crd, fill = \csrd] (gb) circle (1mm) node[yshift=3mm] {\color{\crd}$\omega_2$};
\end{scope}

==> sch/relation_add_dots4.tex <==
\begin{scope}
  \coordinate (m) at (0,0);
  \coordinate (t) at (2,0);
  \draw[->] (m) -- (t) node[pos = 1, right] {$a$} coordinate[pos=0.5] (ga) coordinate[pos=0.7] (gb);
  \filldraw[draw= \crd, fill = \csrd] (ga) circle (1mm) node[yshift= 3mm] {\color{\crd}$\omega_1+\omega_2$};
\end{scope}

==> sch/relation_add_dots6.tex <==
\begin{scope}
  \coordinate (m) at (0,0);
  \coordinate (t) at (2,0);
  \draw[->] (m) -- (t) node[pos = 1, right] {$a$} coordinate[pos=0.5] (ga) node[pos= 0.5 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=1.2pt] {} node[pos=0.5, above, yshift=0.5mm]{\color{\crd}$\omega_1 + \omega_2$};
\end{scope}

==> sch/relation_hollow_black_dots_1.tex <==
\begin{scope}
  \coordinate (m) at (0,0);
  \coordinate (t) at (2,0);
  \draw[->] (m) -- (t) node[pos = 1, right] {$a$} coordinate[pos=0.2] (ga) coordinate[pos=0.8] (gb) coordinate[pos=0.5,yshift=6mm] (gc) coordinate[pos=0.5,yshift=-6mm] (gd);
  \filldraw[draw= \crd, fill = white] (ga) circle (1mm) node[yshift= 3.5mm] {$-\omega$};
  \filldraw[draw= black, fill = black] (gb) circle (1mm) node[yshift=3.5mm] {$\omega$};
\end{scope}

==> sch/relation_hollow_black_dots_2.tex <==
\begin{scope}
  \coordinate (m) at (  0,  0);
  \coordinate (t) at (  2, 0);
  \draw[->] (m) -- (t) node[pos = 1, right] {$a$} coordinate[pos=0.5] (ga);
  \filldraw[draw= \crd, fill = \csrd] (ga) circle (1mm) node[yshift= 3mm] {$\omega$};
\end{scope}

==> sch/theta_blank.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/theta_kl.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw (0:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[right]{$p_k$};
	\draw (180:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[left]{$p_l$};
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/theta_left_kl.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw (180:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[left]{$p_l\hat{p}_k$};
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/theta_right_kl.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw (0:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[right]{$p_l\hat{p}_k$};
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/toruslink_2.tex <==
\begin{scope}[xshift = 2.5cm]

	\draw[-] (0.5, -2.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5,-1.5);
	\fill[white] (0,-2) circle (2mm);
	\draw[-] (-0.5, -2.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5,-1.5);

	\node at (0,-1) {$\cdots$};

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5) .. controls +(0,-0.5) and +(0, 0.5) .. (0.5, -0.5);
	\fill[white] (0, 0) circle (1mm);
	\draw[-] (-0.5, -0.5) .. controls +(0,0.5) and +(0, -0.5) .. (0.5, 0.5);

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s$};

	\draw[->-] (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,-2.5) arc (-180:0:0.5)  ;
	\draw[->-] (0.5, 2) arc (180:0:0.5)  -- (1.5,-2.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/toruslink_4.tex <==
\begin{scope}[xshift = 2.5cm]

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5);

	\draw[-] (0.5,0.5) -- (0.5,-2.5);
	\draw[-] (-0.5,0.5) -- (-0.5,-2.5);

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s+m-1$};

	\draw[->-] (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,-2.5) arc (-180:0:0.5)  ;
	\draw[->-] (0.5, 2) arc (180:0:0.5)  -- (1.5,-2.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/toruslink_5.tex <==
\begin{scope}[xshift = 2.5cm]

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5);

	% \draw[-] (0.5,0.5) -- (0.5,-2.5);
	% \draw[-] (-0.5,0.5) -- (-0.5,-2.5);

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s+m-1$};

	\draw[->-] (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,0.5) arc (-180:0:0.5)  ;
	\draw[->-] (0.5, 2) arc (180:0:0.5)  -- (1.5,0.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/toruslink_5b.tex <==
\begin{scope}[xshift = 2.5cm]

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5);

	% \draw[-] (0.5,0.5) -- (0.5,-2.5);
	% \draw[-] (-0.5,0.5) -- (-0.5,-2.5);

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s+m-2$};

	\draw[->-] (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,0.5) arc (-180:0:0.5)  ;
	\draw[->-] (0.5, 2) arc (180:0:0.5)  -- (1.5,0.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/toruslink_5c.tex <==
\begin{scope}[xshift = 2.5cm]

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5);

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s+1$};

	\draw[->-] (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,0.5) arc (-180:0:0.5)  ;
	\draw[->-] (0.5, 2) arc (180:0:0.5)  -- (1.5,0.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/unframed_1.tex <==
\begin{scope}
   \coordinate (bl) at (-0.5, -1);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (tl) at (-0.5,  1);
    \coordinate (tr) at ( 0.5,  1);
    \draw[->] (bl) -- (tl)  node[pos=0.2, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.2, right]{$\frac{1}{2}$};
    \draw[->] (br) -- (tr);
    \draw[decorate,decoration={snake}] (-1.08,-1.4) -- (1.08,-1.4);
\end{scope}

==> sch/unframed_3.tex <==
\begin{scope}
   \coordinate (bl) at (-0.5, -1);
    \coordinate (br) at ( 0.5, -1);
    \coordinate (tl) at (-0.5,  1);
    \coordinate (tr) at ( 0.5,  1);
    \draw[->] (bl) -- (tl)  node[pos=0.2, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.2, right]{$-\frac{1}{2}$};
    \draw[->] (br) -- (tr);
    \draw[decorate,decoration={snake}] (-1.08,-1.4) -- (1.08,-1.4);
\end{scope}

==> sch/web_associativity1.tex <==
\begin{scope}
  \coordinate (b) at ( 0,-0.50);
  \coordinate (m) at (0,0);
  \coordinate (tr) at (+1,  1);
  \coordinate (tm) at (0,  1);
  \coordinate (tl) at (-1,  1);
  \draw[>-, >= to] (b) -- (m) node[pos=0, below] {$a+b+c$};
  \draw[-to] (m) .. controls +(0,0) and + (0, -0.5) .. (tl) node[pos =
  1, above] {$a$} coordinate[pos= 0.5] (ml) coordinate[pos = 0.25] (lml);
  \draw[-to] (m) .. controls +(0,0) and + (0, -0.5) .. (tr) node[pos =
  1, above] {$c$};
  \draw[-to] (ml)  .. controls +(0,0) and + (0, -0.5) .. (tm) node[pos =
  1, above] {$b$};
\end{scope}

==> sch/web_associativity2.tex <==
\begin{scope}
  \coordinate (b) at ( 0,-0.50);
  \coordinate (m) at (0,0);
  \coordinate (tr) at (+1,  1);
  \coordinate (tm) at (0,  1);
  \coordinate (tl) at (-1,  1);
  \draw[>-, >= to] (b) -- (m) node[pos=0, below] {$a+b+c$};
  \draw[-to] (m) .. controls +(0,0) and + (0, -0.5) .. (tl) node[pos =
  1, above] {$c$} coordinate[pos= 0.5] (ml) coordinate[pos = 0.25] (lml);
  \draw[-to] (m) .. controls +(0,0) and + (0, -0.5) .. (tr) node[pos =
  1, above] {$a$};
  \draw[-to] (ml)  .. controls +(0,0) and + (0, -0.5) .. (tm) node[pos =
  1, above] {$b$};
\end{scope}

==> sch/web_associativity3.tex <==
\begin{scope}
  \coordinate (t) at ( 0,0.50);
  \coordinate (m) at (0,0);
  \coordinate (br) at (+1,  -1);
  \coordinate (bm) at ( 0,  -1);
  \coordinate (bl) at (-1,  -1);
  \draw[-to] (m) -- (t) node[pos=1, above] {$a+b+c$};
  \draw[>-, >=to] (bl) .. controls +(0,0.5) and + (0, 0) .. (m) node[pos =
  0, below] {$a$} coordinate[pos= 0.5] (ml) coordinate[pos = 0.75] (lml);
  \draw[>-, >=to] (br) .. controls +(0,0.5) and + (0, -0) .. (m) node[pos =
  0, below] {$c$};
  \draw[>-, >=to] (bm)  .. controls +(0,0.5) and + (0, 0) .. (ml) node[pos =
  0, below] {$b$};
\end{scope}

==> sch/web_circle_cap.tex <==
\begin{scope}[scale= 1]
  \draw[->] (0,0) arc (0:360: 0.8) node[pos=1, right] {$a$} coordinate[pos=0.45]
  (ga); 
  \filldraw[draw= \crd, fill = \csrd] (ga) circle (1mm)
  node[left, black] {$-\frac{1}{2}$};
\end{scope}

==> sch/web_circle_cup.tex <==
\begin{scope}[scale= 1]
  \draw[->] (0,0) arc (0:360: 0.8) node[pos=1, right] {$a$} coordinate[pos=0.45]
  (ga); 
  \filldraw[draw= \crd, fill = \csrd] (ga) circle (1mm)
  node[left, black] {$\frac{1}{2}$};
\end{scope}

==> sch/web_digon.tex <==
\begin{scope}
  \coordinate (bm) at ( 0, -1);
  \coordinate (cm) at ( 0, -0.6);
  \coordinate (sm) at ( 0,  0.6);
  \coordinate (tm) at ( 0, 1);
  \draw[dotted] (0,0) circle (1);
  \draw[->] (sm) -- (tm) node[above, pos =1] {$a+b$};
  \draw[->-] (cm) .. controls + ( 0.6, 0.6) and + ( 0.6, -0.6) .. (sm)
  node [pos = 0.5, right] {$b$}  ;
  \draw[->-] (cm) .. controls + (-0.6, 0.6) and + (-0.6, -0.6) .. (sm)
  node [pos = 0.5,  left] {$a$};
  \draw[] (bm) -- (cm) node[pos=0, below] {$a+b$};
\end{scope}

==> sch/web_digoncap_beg.tex <==
\begin{scope}
  \coordinate (bm) at ( 0, -1);
  \coordinate (cm) at ( 0, -0.6);
  \coordinate (sm) at ( 0,  0.6);
  \coordinate (tm) at ( 0, 1);
  \draw[->] (sm) -- (tm) node[above, pos =1] {$a+b$};
  \draw[->-] (cm) .. controls + ( 0.6, 0.6) and + ( 0.6, -0.6) .. (sm)
  node [pos = 0.5, right] {$b$} node[pos= 0.8 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.8, right]{$a\mu$}; ;
  \draw[->-] (cm) .. controls + (-0.6, 0.6) and + (-0.6, -0.6) .. (sm)
  node [pos = 0.5,  left] {$a$} node[pos= 0.8 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.8, left]{$b\lambda$};
  \draw[>-] (bm) -- (cm) node[below, pos =0] {$a+b$} node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1, right]{$-\bar{s}$} ;
\end{scope}

==> sch/web_digoncup_end.tex <==
\begin{scope}
  \coordinate (bm) at ( 0, -1);
  \coordinate (cm) at ( 0, -0.6);
  \coordinate (sm) at ( 0,  0.6);
  \coordinate (tm) at ( 0, 1);
  \draw[->] (sm) -- (tm) node[above, pos =1] {$a+b$};
  \draw[->-] (cm) .. controls + ( 0.6, 0.6) and + ( 0.6, -0.6) .. (sm)
  node [pos = 0.5, right] {$b$} node[pos= 0.8 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.8, right]{$a\mu$}; ;
  \draw[->-] (cm) .. controls + (-0.6, 0.6) and + (-0.6, -0.6) .. (sm)
  node [pos = 0.5,  left] {$a$} node[pos= 0.8 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.8, left]{$b\lambda$};
  \draw[>-] (bm) -- (cm) node[below, pos =0] {$a+b$} node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1, right]{$s$} ;
\end{scope}

==> sch/web_l_ab.tex <==
\begin{scope}
  \coordinate (bm) at ( 0, -1);
  \coordinate (tm) at ( 0, 1);
  \draw[>->] (bm) -- (tm) node[above, pos =1] {$a+b$} node[below, pos =0] {$a+b$};
\end{scope}

==> sch/web_saddle_a_beg.tex <==
\begin{scope}[scale= 1]
  \draw [->] (45:0.8) arc (-45:-135:0.8) node [pos=1, above] {$a$};
  \draw [<-] (-45:0.8) arc (45: 135:0.8) node [pos=0, below] {$a$};
\end{scope}

==> sch/web_saddle_a_end.tex <==
\begin{scope}[scale= 1]
    \draw [->] (45:0.8) arc (135:225:0.8) coordinate[pos=0.5] (ga) node [pos=1, below] {$a$};
    \draw [<-] (135:0.8) arc (-135:-225:-0.8) node [pos=0, above] {$a$};
    \filldraw[draw= \crd, fill = \csrd] (ga) circle (1mm) node[right, black] {$-\frac{1}{2}$};
\end{scope}





==> sch/zero_cohomo.tex <==
\begin{scope}
  \coordinate (bl) at (-0.5, -1);
  \coordinate (br) at ( 0.5, -1);
  \coordinate (bm) at (  0,-0.3);
  \coordinate (tl) at (-0.5,  1);
  \coordinate (tr) at ( 0.5,  1);
  \coordinate (tm) at (  0, 0.3);
  \draw[>-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[>-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[<-]  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw[<-]  (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw [double] (bm) -- (tm);
\end{scope}
